RNA: Relightable Neural Assets

High-fidelity 3D assets with materials composed of fibers (including hair), complex layered material shaders, or fine scattering geometry are ubiquitous in high-end realistic rendering applications. Rendering such models is computationally expensive due to heavy shaders and long scattering paths. Moreover, implementing the shading and scattering models is non-trivial and has to be done not only in the 3D content authoring software (which is necessarily complex), but also in all downstream rendering solutions. For example, web and mobile viewers for complex 3D assets are desirable, but frequently cannot support the full shading complexity allowed by the authoring application. Our goal is to design a neural representation for 3D assets with complex shading that supports full relightability and full integration into existing renderers. We provide an end-to-end shading solution at the first intersection of a ray with the underlying geometry. All shading and scattering is precomputed and included in the neural asset; no multiple scattering paths need to be traced, and no complex shading models need to be implemented to render our assets, beyond a single neural architecture. We combine an MLP decoder with a feature grid. Shading consists of querying a feature vector, followed by an MLP evaluation producing the final reflectance value. Our method provides high-fidelity shading, close to the ground-truth Monte Carlo estimate even at close-up views. We believe our neural assets could be used in practical renderers, providing significant speed-ups and simplifying renderer implementations.

==> chapters/performance.tex <==
% !TEX root = ../main.tex

\section{Performance}
\label{sec:performance}

We use a Windows 11 workstation that has an AMD Threadripper 3990X 64 core CPU for all the rendering results shown. The 
We tested our rendering performance on a Windows 11 desktop running Ubuntu through Windows Subsystem for Linux (WSL) with an AMD Threadripper 3990x CPU (64 cores), Nvidia RTX A6000 GPU (48GB VRAM) and 128GB of RAM.
As detailed in the previous section, our implementation renders by tracing primary rays on the CPU and shading on the GPU.
All images with our model are rendered with a resolution of $1024^2$ and $16$ samples per pixel.
We benchmark the performance to render the human hair asset shown in \figref{fig:teaser}: the primary ray tracing on CPU using Cycles takes $18.5$ seconds, including time to read and write the deep buffers to disk, while the shading on GPU takes $5.5$ seconds.
This is many times faster than the Monte Carlo reference method; to get an equivalent quality with Cycles on the CPU at 256 samples per pixel, it takes $210$ seconds with some residual noise remaining.

